Thematic Domain Analysis for Ocean Modeling

Ocean science is a discipline that employs ocean models as an essential research asset. Such scientific modeling provides mathematical abstractions of real-world systems, e.g., the oceans. These models are then coded as implementations of the mathematical abstractions. The developed software systems are called models of the real-world system. To advance the state in engineering such ocean models, we intend to better understand how ocean models are developed and maintained in ocean science. In this paper, we present the results of semi-structured interviews and the Thematic Analysis~(TA) of the interview results to analyze the domain of ocean modeling. Thereby, we identified developer requirements and impediments to model development and evolution, and related themes. This analysis can help to understand where methods from software engineering should be introduced and which challenges need to be addressed. We suggest that other researchers extend and repeat our TA with model developers and research software engineers working in related domains to further advance our knowledge and skills in scientific modeling.

==> sec-interview-setup.tex <==
\section{Interviews}

We conducted the interviews primarily in the office of the scientists and technical staff to increase the convenience for the interviewees. 
However, in some cases we deviated from this setup, as interviewees did not want to disturb other people in their office.
Also, due to the SARS-CoV-2 crisis, the later interviews were conducted by video conference.
All interviews were recorded and later transcribed.

As we used semi-structured expert interviews, we developed an interview guide addressing the context and background of the interviewees, their work process, the technical environment they work in, and whether they use software engineering methods.

\paragraph{Demographics}
The interview starts with questions concerning the scope of interviewees' jobs, e.g., scientist or technical staff, their research interest, and background.
This is necessary to understand the involved disciplines and topics addressed within the domain.

\paragraph{Work Process}
The first main questions address how people work in ocean modeling.
Here we where interested primarily in their work processes and interactions with others during modeling.
This includes all processes and steps the interviewees perform before they start using and modifying models.

\paragraph{Tool Environment}
The second block addressed the software and tool environment they use to develop, test, and run their models.
This is important, as the acceptance of new tools and practices depends on the ability to use them with little effort.

\paragraph{Software Engineering Methods}
The interview closed with questions regarding software engineering methods, such as testing, code checker, and feature management.
 

==> sec-related-work.tex <==
\section{Related Work}

\todo[inline]{Fehlt noch}

In recent years the qualitative research method grounded theory has found its way into software engineering.
Unfortunately, grounded theory is not used in the right way in most publications that state to use it;
instead some associated techniques are used without engaging the whole methodology \citep{Stol2016}.
This removes the advantage of an established approach to control analysis and quality assurance.
In addition, grounded theory aims to establish new concepts and ideas based on a data set, e.g., interview transcripts, working without using a distinct research question during the analysis.
However, our semi-structured interview is based on a key research question and specific interview questions.
Therefore, we decided us against using grounded theory and instead use a method better fitting to our data set comprising of semi-structured interviews, called Thematic Analysis~(TA).

